Deep Video Restoration for Under-Display Camera

Images or videos captured by the Under-Display Camera (UDC) suffer from severe degradation, such as saturation degeneration and color shift. While restoration for UDC has been a critical task, existing works of UDC restoration focus only on images. UDC video restoration (UDC-VR) has not been explored in the community. In this work, we first propose a GAN-based generation pipeline to simulate the realistic UDC degradation process. With the pipeline, we build the first large-scale UDC video restoration dataset called PexelsUDC, which includes two subsets named PexelsUDC-T and PexelsUDC-P corresponding to different displays for UDC. Using the proposed dataset, we conduct extensive benchmark studies on existing video restoration methods and observe their limitations on the UDC-VR task. To this end, we propose a novel transformer-based baseline method that adaptively enhances degraded videos. The key components of the method are a spatial branch with local-aware transformers, a temporal branch embedded temporal transformers, and a spatial-temporal fusion module. These components drive the model to fully exploit spatial and temporal information for UDC-VR. Extensive experiments show that our method achieves state-of-the-art performance on PexelsUDC. The benchmark and the baseline method are expected to promote the progress of UDC-VR in the community, which will be made public.

==> figures/cake.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/cake.pdf}
    \caption{(a) Category proportion of video contents in {\dataset}. About half of the videos contain people or animals. The other half includes non-living objects or scenes. (b) The proportion of different degrees of camera movements in videos of {\dataset}. Two-thirds of the videos have obvious camera movements, and the remaining videos contain slight or few camera movements.}
    \label{fig: cake}
    \vspace{-0.4cm}
\end{figure}


==> figures/collection_pipeline.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/workflow.pdf}
    \caption{UDC video generation pipeline (UVGP) for {\dataset}. Almost half of videos are eliminated due to unsatisfactory quality before stage 2. Around 83.9 percent of generated videos are excluded from the final {\dataset} for the purpose of eliminating artifacts and making the categories balanced.} \label{fig:collection}
\end{figure}

==> figures/p_gen_results.tex <==
\begin{figure*}[t] \centering
    \includegraphics[width=0.95\textwidth]{images/p_gen_results.pdf}
    \caption{Generation comparison on POLED \cite{zhou2021image} dataset. *DAGF \cite{sundar2020deep} is trained on misaligned data and we follow its way for image generation.}
    \label{fig: p_gen_results}
\end{figure*}


==> figures/t_gen_results.tex <==
\begin{figure*}[t] \centering
    \includegraphics[width=0.95\textwidth]{t_gen_results.pdf}
    \caption{Generation comparison on TOLED \cite{zhou2021image} dataset. *DAGF is trained on misaligned data and we follow its way for image generation.}
    \label{fig: t_gen_results}
\end{figure*}


==> tables/ablation_window.tex <==
\begin{table}[ht]
    \centering
    \caption{Ablation studies on the window size of Temporal Transformer.}
    \vspace{-0.2cm}
    \scalebox{0.80}{
        \setlength{\tabcolsep}{4mm}{
            \begin{tabular}{|c|cccc|}
                \cline{1-5}
                Window size & $1\times 1$ & $2\times 2$ &  $4\times 4$ & $8\times 8$ \\
                \cline{1-5}
                PSNR$\uparrow$ & 32.90 & 32.98   & \textbf{33.59}  & 33.05  \\ 
                SSIM$\uparrow$ & 0.9108 & 0.9130 & \textbf{0.9193} & 0.9135  \\
                \cline{1-5}
            \end{tabular}
        }
    }
    \label{tab: win_size}
\end{table}


==> tables/gen_results.tex <==
\begin{table*}[t]
    \centering
    \newcommand{\Frst}[1]{\textcolor{red}{\textbf{#1}}}
    \newcommand{\Scnd}[1]{\textcolor{blue}{\textbf{#1}}}
    % \newcommand{\Frst}[1]{\textcolor{red}{\textbf{#1}}}
    % \newcommand{\Scnd}[1]{\underline{\textbf{#1}}
    \newcommand{\psnr}{PSNR$\uparrow$}
    \newcommand{\ssim}{SSIM$\uparrow$}
    \newcommand{\lpips}{LPIPS$\downarrow$}
    \newcommand{\dists}{DISTS$\downarrow$}
  
    \caption{Results of generation on TOLED and POLED \cite{zhou2021image} validation datasets. The best and second-best results are marked in bold and underlined respectively. $\uparrow$ means the higher value is better. $\downarrow$ means the lower value is better.}
    \begin{tabular}{|l|*{2}{c}*{2}{c}|*{2}{c}*{2}{c}|}
        \cline{1-9}
        \multirow{2}*{Methods} & \multicolumn{4}{c|}{\textbf{TOLED}} & \multicolumn{4}{c|}{\textbf{POLED}} \\
        \cline{2-9}
        % \toprule
        & \psnr & \ssim & \lpips & \dists & \psnr & \ssim & \lpips & \dists \\
        \cline{1-9}
        % DAGF*~\cite{sundar2020deep} & 18.9890 & 0.7039 & 0.5786 & 0.3065 & 34.3726 & \Scnd{0.9158} & 0.5100 & 0.3110 \\
        % DAGF*~\cite{sundar2020deep} & - & - & - & - & - & - & - & - \\
        % \cline{1-9}
        MPGNet~\cite{zhou2022modular} & 31.9882 & 0.8728 & 0.3702 & 0.2128 & 32.4927 & \underline{0.8719} & \underline{0.3171} & \underline{0.1181} \\
        \textbf{Ours (w/o noise)} & \textbf{35.2854} & \textbf{0.9455} & \underline{0.2739} & \underline{0.1616} & \textbf{37.3177} & \textbf{0.9268} & 0.3562  & 0.2143 \\
        \textbf{Ours} & \underline{34.7756} & \underline{0.9233} & \textbf{0.2183} & \textbf{0.0863} & \underline{35.5063} & 0.8694 & \textbf{0.3024} & \textbf{0.1011}\\ 
        \cline{1-9}
    \end{tabular}
    \label{tab: generation}
\end{table*}
